Downtime Optimized Live Migration of Industrial Real-Time Control Services

Live migration of services is a prerequisite for various use cases that must be fulfilled for the realization of Industry 4.0. In addition, many different types of services need to provide mobility and consequently need to be migrated live. These can be offloaded algorithms from mobile devices, such as unmanned vehicles or robots, security services, communication services or classic control tasks. In particular, the latter place very high demands on determinism and latency. Here, it is of utmost importance that the downtime of the service is as low as possible. Since existing live migration approaches try to optimize multiple metrics such as downtime, migration time as well as energy consumption, which are equally relevant in the IT domain, it is not possible to use any of these approaches without adoptions. Therefore, a novel concept is proposed that builds on top of both existing migration approaches as well as virtualization technologies and aims primarily at minimizing service downtime. Furthermore, the concept is evaluated using a test environment. The results show that a sub-millisecond downtime can be achieved with the proposed concept. Moreover, the total migration time is in the range of several hundred milliseconds for the highest performance setting and two seconds for a non-invasive approach.

==> organization/IEEE_authors.tex <==
% author names and affiliations
% use a multiple column layout for up to three different
% affiliations
\author{%
%
\IEEEauthorblockN{%
    Michael Gundall\IEEEauthorrefmark{1},\\%
    %Christoph Fischer\IEEEauthorrefmark{2}%
}
\IEEEauthorblockA{%
    German Research Center for\\Artificial Intelligence GmbH, DFKI\\%
    Trippstadter Str. 122\\%
    67663 Kaiserslautern\\%
    Email: %{\tt
      \{%
        \IEEEauthorrefmark{1}dennis.krummacker,\\%
        \hspace*{1em}\IEEEauthorrefmark{2}christoph.fischer%
      \}@dfki.de
    %}%
}
%
\and%
%
\IEEEauthorblockN{%
    FirstName1 Lastname1\IEEEauthorrefmark{3},\\%
    FirstName2 Lastname2\IEEEauthorrefmark{4}
}%
\IEEEauthorblockA{%
	Chair of Something\\
    Faculty of Amazing Computer Science\\
    University\\
    Optional Address\\
    Email: \{\IEEEauthorrefmark{3}Mail1,\\ \hspace*{1em}\IEEEauthorrefmark{4}Mail2\}@domain.de
}%
}%
%
%








% conference papers do not typically use \thanks and this command
% is locked out in conference mode. If really needed, such as for
% the acknowledgment of grants, issue a \IEEEoverridecommandlockouts
% after \documentclass

% for over three affiliations, or if they all won't fit within the width
% of the page, use this alternative format:
% 
%\author{\IEEEauthorblockN{Michael Shell\IEEEauthorrefmark{1},
%Homer Simpson\IEEEauthorrefmark{2},
%James Kirk\IEEEauthorrefmark{3}, 
%Montgomery Scott\IEEEauthorrefmark{3} and
%Eldon Tyrell\IEEEauthorrefmark{4}}
%\IEEEauthorblockA{\IEEEauthorrefmark{1}School of Electrical and Computer Engineering\\
%Georgia Institute of Technology,
%Atlanta, Georgia 30332--0250\\ Email: see http://www.michaelshell.org/contact.html}
%\IEEEauthorblockA{\IEEEauthorrefmark{2}Twentieth Century Fox, Springfield, USA\\
%Email: homer@thesimpsons.com}
%\IEEEauthorblockA{\IEEEauthorrefmark{3}Starfleet Academy, San Francisco, California 96678-2391\\
%Telephone: (800) 555--1212, Fax: (888) 555--1212}
%\IEEEauthorblockA{\IEEEauthorrefmark{4}Tyrell Inc., 123 Replicant Street, Los Angeles, California 90210--4321}}





==> organization/_templates/IEEE_authors-long.tex <==
% author names and affiliations
% use a multiple column layout for up to three different
% affiliations
\author{%
%
\IEEEauthorblockN{%
    Dennis Krummacker\IEEEauthorrefmark{1}, %
    Christoph Fischer\IEEEauthorrefmark{2}, %
    \\%
    FirstName1 Lastname1\IEEEauthorrefmark{3} and %
    FirstName2 Lastname2\IEEEauthorrefmark{4}%
}%
\IEEEauthorblockA{%
    \IEEEauthorrefmark{1}\IEEEauthorrefmark{2}German Research Center for Artificial Intelligence GmbH (DFKI)%
%     Trippstadter Str. 122\\%
%     67663 Kaiserslautern\\%
	\\%
    \IEEEauthorrefmark{3}Institute1, %
    Some Subtitle 1 %
%     Optional Address, Germany%
    \\%
	\IEEEauthorrefmark{4}Corporation2, %
    Some Subtitle2, %
    Some more Subt2 %
%     Optional Address
    \\%
    Email: %
        \{\IEEEauthorrefmark{1}dennis.krummacker, %
        \IEEEauthorrefmark{2}christoph.fischer\}@dfki.de, %
        \\%
        \IEEEauthorrefmark{3}Mail1@domain1.de, %
        \IEEEauthorrefmark{4}Mail2@domain2.com
}%
}%






% conference papers do not typically use \thanks and this command
% is locked out in conference mode. If really needed, such as for
% the acknowledgment of grants, issue a \IEEEoverridecommandlockouts
% after \documentclass

% for over three affiliations, or if they all won't fit within the width
% of the page, use this alternative format:
% 
%\author{\IEEEauthorblockN{Michael Shell\IEEEauthorrefmark{1},
%Homer Simpson\IEEEauthorrefmark{2},
%James Kirk\IEEEauthorrefmark{3}, 
%Montgomery Scott\IEEEauthorrefmark{3} and
%Eldon Tyrell\IEEEauthorrefmark{4}}
%\IEEEauthorblockA{\IEEEauthorrefmark{1}School of Electrical and Computer Engineering\\
%Georgia Institute of Technology,
%Atlanta, Georgia 30332--0250\\ Email: see http://www.michaelshell.org/contact.html}
%\IEEEauthorblockA{\IEEEauthorrefmark{2}Twentieth Century Fox, Springfield, USA\\
%Email: homer@thesimpsons.com}
%\IEEEauthorblockA{\IEEEauthorrefmark{3}Starfleet Academy, San Francisco, California 96678-2391\\
%Telephone: (800) 555--1212, Fax: (888) 555--1212}
%\IEEEauthorblockA{\IEEEauthorrefmark{4}Tyrell Inc., 123 Replicant Street, Los Angeles, California 90210--4321}}





==> organization/_templates/IEEE_authors.tex <==
% author names and affiliations
% use a multiple column layout for up to three different
% affiliations
\author{%
%
\IEEEauthorblockN{%
    Dennis Krummacker\IEEEauthorrefmark{1},\\%
    Christoph Fischer\IEEEauthorrefmark{2}%
}
\IEEEauthorblockA{%
    German Research Center for\\Artificial Intelligence GmbH, DFKI\\%
    Trippstadter Str. 122\\%
    67663 Kaiserslautern\\%
    Email: %{\tt
      \{%
        \IEEEauthorrefmark{1}dennis.krummacker,\\%
        \hspace*{1em}\IEEEauthorrefmark{2}christoph.fischer%
      \}@dfki.de
    %}%
}
%
\and%
%
\IEEEauthorblockN{%
    FirstName1 Lastname1\IEEEauthorrefmark{3},\\%
    FirstName2 Lastname2\IEEEauthorrefmark{4}
}%
\IEEEauthorblockA{%
	Chair of Something\\
    Faculty of Amazing Computer Science\\
    University\\
    Optional Address\\
    Email: \{\IEEEauthorrefmark{3}Mail1,\\ \hspace*{1em}\IEEEauthorrefmark{4}Mail2\}@domain.de
}%
}%
%
%









%\author{%
%           \IEEEauthorblockN{Michael Shell}
%           \IEEEauthorblockA{School of Electrical and\\Computer Engineering\\
%           Georgia Institute of Technology\\
%           Atlanta, Georgia 30332--0250\\
%           Email: http://www.michaelshell.org/contact.html}
%           \and
%           \IEEEauthorblockN{Homer Simpson}
%           \IEEEauthorblockA{Twentieth Century Fox\\
%           Springfield, USA\\
%           Email: homer@thesimpsons.com}
%           \and
%           \IEEEauthorblockN{James Kirk\\ and Montgomery Scott}
%           \IEEEauthorblockA{Starfleet Academy\\
%           San Francisco, California 96678--2391\\
%           Telephone: (800) 555--1212\\
%           Fax: (888) 555--1212}
%
%}%

% conference papers do not typically use \thanks and this command
% is locked out in conference mode. If really needed, such as for
% the acknowledgment of grants, issue a \IEEEoverridecommandlockouts
% after \documentclass

% for over three affiliations, or if they all won't fit within the width
% of the page, use this alternative format:
% 
%\author{\IEEEauthorblockN{Michael Shell\IEEEauthorrefmark{1},
%Homer Simpson\IEEEauthorrefmark{2},
%James Kirk\IEEEauthorrefmark{3}, 
%Montgomery Scott\IEEEauthorrefmark{3} and
%Eldon Tyrell\IEEEauthorrefmark{4}}
%\IEEEauthorblockA{\IEEEauthorrefmark{1}School of Electrical and Computer Engineering\\
%Georgia Institute of Technology,
%Atlanta, Georgia 30332--0250\\ Email: see http://www.michaelshell.org/contact.html}
%\IEEEauthorblockA{\IEEEauthorrefmark{2}Twentieth Century Fox, Springfield, USA\\
%Email: homer@thesimpsons.com}
%\IEEEauthorblockA{\IEEEauthorrefmark{3}Starfleet Academy, San Francisco, California 96678-2391\\
%Telephone: (800) 555--1212, Fax: (888) 555--1212}
%\IEEEauthorblockA{\IEEEauthorrefmark{4}Tyrell Inc., 123 Replicant Street, Los Angeles, California 90210--4321}}





==> organization/backing/IEEETemplateProvidedExamples.tex <==
% An example of a floating figure using the graphicx package.
% Note that \label must occur AFTER (or within) \caption.
% For figures, \caption should occur after the \includegraphics.
% Note that IEEEtran v1.7 and later has special internal code that
% is designed to preserve the operation of \label within \caption
% even when the captionsoff option is in effect. However, because
% of issues like this, it may be the safest practice to put all your
% \label just after \caption rather than within \caption{}.
%
% Reminder: the "draftcls" or "draftclsnofoot", not "draft", class
% option should be used if it is desired that the figures are to be
% displayed while in draft mode.
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=2.5in]{myfigure}
% where an .eps filename suffix will be assumed under latex, 
% and a .pdf suffix will be assumed for pdflatex; or what has been declared
% via \DeclareGraphicsExtensions.
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure}

% Note that the IEEE typically puts floats only at the top, even when this
% results in a large percentage of a column being occupied by floats.


% An example of a double column floating figure using two subfigures.
% (The subfig.sty package must be loaded for this to work.)
% The subfigure \label commands are set within each subfloat command,
% and the \label for the overall figure must come after \caption.
% \hfil is used as a separator to get equal spacing.
% Watch out that the combined width of all the subfigures on a 
% line do not exceed the text width or a line break will occur.
%
%\begin{figure*}[!t]
%\centering
%\subfloat[Case I]{\includegraphics[width=2.5in]{box}%
%\label{fig_first_case}}
%\hfil
%\subfloat[Case II]{\includegraphics[width=2.5in]{box}%
%\label{fig_second_case}}
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure*}
%
% Note that often IEEE papers with subfigures do not employ subfigure
% captions (using the optional argument to \subfloat[]), but instead will
% reference/describe all of them (a), (b), etc., within the main caption.
% Be aware that for subfig.sty to generate the (a), (b), etc., subfigure
% labels, the optional argument to \subfloat must be present. If a
% subcaption is not desired, just leave its contents blank,
% e.g., \subfloat[].


% An example of a floating table. Note that, for IEEE style tables, the
% \caption command should come BEFORE the table and, given that table
% captions serve much like titles, are usually capitalized except for words
% such as a, an, and, as, at, but, by, for, in, nor, of, on, or, the, to
% and up, which are usually not capitalized unless they are the first or
% last word of the caption. Table text will default to \footnotesize as
% the IEEE normally uses this smaller font for tables.
% The \label must come after \caption as always.
%
% \begin{table}[!t]
% % increase table row spacing, adjust to taste
% \renewcommand{\arraystretch}{1.3}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
% \caption{An Example of a Table}
% \label{table_example}
% \centering
% % Some packages, such as MDW tools, offer better commands for making tables
% % than the plain LaTeX2e tabular which is used here.
% \begin{tabular}{|c||c|}
% \hline
% One & Two\\
% \hline
% Three & Four\\
% \hline
% \end{tabular}
% \end{table}

==> organization/backing/thebibliography.tex <==
% can use a bibliography generated by BibTeX as a .bbl file
% BibTeX documentation can be easily obtained at:
% http://mirror.ctan.org/biblio/bibtex/contrib/doc/
% The IEEEtran BibTeX style support page is at:
% http://www.michaelshell.org/tex/ieeetran/bibtex/
%\bibliographystyle{IEEEtran}
% argument is your BibTeX string definitions and bibliography database(s)
%\bibliography{IEEEabrv,../bib/paper}
%
% <OR> manually copy in the resultant .bbl file
% set second argument of \begin to the number of references
% (used to reserve space for the reference number labels box)
\begin{thebibliography}{1}

\bibitem{IEEEhowto:kopka}
H.~Kopka and P.~W. Daly, \emph{A Guide to \LaTeX}, 3rd~ed.\hskip 1em plus
  0.5em minus 0.4em\relax Harlow, England: Addison-Wesley, 1999.
  
\bibitem{IEC61158}
, \emph{IEC 61158},

\bibitem{61158-trafficclass}
E DIN EN 61158-1:2017-09 11.4.2

\bibitem{61158-endpoint}
E DIN EN 61158-1:2017-09 9.3.3.3.1

\bibitem{62439-endnode}
DIN EN 62439-1:2010-09 3.1.13

\end{thebibliography}
